A Sound and Complete Hoare Logic for Dynamically-Typed, Object-Oriented Programs -- Extended Version --

A simple dynamically-typed, (purely) object-oriented language is defined. A structural operational semantics as well as a Hoare-style program logic for reasoning about programs in the language in multiple notions of correctness are given. The Hoare logic is proved to be both sound and (relative) complete and is -- to the best of our knowledge -- the first such logic presented for a dynamically-typed language.

==> sections/dyn_and_stat.tex <==
\newcommand{\textPL}[1]{\textsl{#1}}

%\section{Dynamically Typed Languages}

%\subsection{Dynamically Typed Model Language: dyn}

To present our methodology we need a pair of programming languages that differ only in the fact that one
is dynamically typed wile the other uses a static type system. Although such pairings exist (JavaScript
and TypeScript for example), we decided to introduce a pair of model languages (called \textbf{dyn} and
\textbf{stat}) to facilitate formal proof.

Designed to resemble their popular real-world siblings, the two are
imperative, class-based object-oriented languages including typical features like inheritance, method
renaming, dynamic dispatch and constructors. However, in order to concentrate on the aspect of dynamic
typing, they do not support advanced dynamic features like a dynamic class hierarchy, method update
or eval().

%
\begin{figure}

% first column
\underline{Syntax of \textbf{dyn}:}

$\mathit{Prog_d} \ni \pi ::= \Vector{\mathit{class}} \PL{ } s$

$\mathit{Class_d} \ni \mathit{class} ::= \PL{class C $<$ C }\{ \Vector{\mathit{meth}} \}$

$\mathit{Meth_d} \ni \mathit{meth} ::= \PL{method m}(\Vector{\PL{u}}) \{ s \} \mid \PL{rename m m}$

$\mathit{Stmt_d} \ni s ::= s;s \mid e$

$\mathit{Expr_d} \ni e ::= \PL{null} \mid \PL{u} \mid \PL{@v} \mid \PL{this} \mid e == e \mid e \PL{ is\_a? C} \mid e.\PL{m}(\Vector{e}) \mid \PL{new C}(\Vector{e})$

\hspace*{0.8cm}$\mid \PL{u} := e \mid \PL{@v} := e \mid \PL{if } e \PL{ then } s \PL{ else } s \PL{ end}\mid \PL{while } e \PL{ do } s \PL{ done}$

$\PL{u} \in \Var_L, \PL{@v} \in \Var_I, \PL{C} \in \Class, \PL{m} \in \Method$

\underline{Syntax of \textbf{stat}:}

\textbf{Stat} is syntactically equivalent to \textbf{dyn}, except for expressions:

$\mathit{Expr_s} \ni e ::= e_{\pure} \mid \PL{u} := e_{\pure}.\PL{m}(\Vector{e_{\pure}}) \mid \PL{u} := \PL{new C}(\Vector{e_{\pure}}) \mid \PL{u} := e_{\pure} \mid \PL{@v} := e_{\pure}$

\hspace*{0.8cm}$\mid \PL{if } e_{\pure} \PL{ then } s \PL{ else } s \PL{ end}\mid \PL{while } e_{\pure} \PL{ do } s \PL{ done}$

$\mathit{Expr_{\pure}} \ni e_{\pure} ::= \PL{null} \mid \PL{u} \mid \PL{@v} \mid \PL{this} \mid e_{\pure} == e_{\pure} \mid e \PL{ is\_a? C} \mid c_{\pure} \mid \mathit{op}(\Vector{e_{\pure}})$

\hspace*{0.8cm}$\mid \PL{if } e_{\pure} \PL{ then } e_{\pure} \PL{ else } e_{\pure} \PL{ end}$

$c_{\pure} \in \mathit{Cnst_s}, \mathit{op}(\Vector{e_{\pure}}) \in \mathit{Op_s}$

\begin{minipage}{0.5\textwidth}
\underline{Syntactic sugar in \textbf{dyn}:} 

$e_1 \oplus e_2 \equiv e_1.\PL{m}_{\oplus}(e_2)$

$\PL{if } e \PL{ then } s \PL{ end} \equiv$

\hspace{1cm}$\PL{if } e \PL{ then } s \PL{ else null end}$

$\mathit{false} \equiv \PL{new bool(null)}$

$\mathit{true} \equiv \mathit{false}.\PL{not()}$

$0 \equiv \PL{new num(null)}$, $n \equiv \PL{$(n-1)$.succ()}$

$"" \equiv \PL{new string(null, null)}$,

$\PL{"...a"} \equiv \PL{"..."}.\PL{addchar}(n_{\PL{a}})$
where $n_{\PL{a}} \in \mathbb{N}$ is the ASCII-code of character $\PL{a}$.
\end{minipage}
\begin{minipage}{0.5\textwidth}
\underline{Basic data types in \textbf{stat}:}

$\mathit{true}, \mathit{false} \in \mathit{Cnst_s}$

$\wedge, \vee, \rightarrow: \mathbb{B} \times \mathbb{B} \mapsto \mathbb{B}  \in \mathit{Op_s}$

$0,1,... \in \mathit{Cnst_s}$

$+,*,div: \mathbb{N} \times \mathbb{N} \mapsto \mathbb{N} \in \mathit{Op_s}$

$=: \mathbb{N} \times \mathbb{N} \mapsto \mathbb{B} \in \mathit{Op_s}$

$"", "a", ... \in \mathit{Cnst_s}$

$+: \mathbb{S} \times \mathbb{S} \mapsto \mathbb{S} \in \mathit{Op_s}$

$s[n]: \mathbb{S} \times \mathbb{N} \mapsto \mathbb{N} \in \mathit{Op_s}$

$|s|: \mathbb{S} \mapsto \mathbb{N} \in \mathit{Op_s}$

\end{minipage}

\caption{\label{fig:lang_syntax}Syntax of \textbf{dyn} and \textbf{stat}}
\end{figure}
\todo{$e==e$ and $e \PL{ is\_a? C}$ were added. Also add to semantics, etc.}


\begin{figure}
Mapping Dyn Types to Stat Types

$\Psi: \mathcal{T}_d \mapsto \mathcal{T}_s$

$\Psi(T) = \begin{cases}
            \mathit{Null} & \text{if } T = \{\}, \\
            \mathbb{N} & \text{if } T = \{\mathit{num}\}, \\
            \mathbb{B} & \text{if } T = \{\mathit{bool}\}, \\
            \mathbb{L} & \text{if } T = \{\mathit{list}\}, \\
            \mathbb{O} & \text{else}
           \end{cases}
$

Predicate for pure expressions:

$\ppure: \mathcal{T}_s \times \mathit{Expr_d} \mapsto \mathbb{B}$

$\ppure(\mathit{Null}, \PL{null}) \equiv \mathit{true}$

$\ppure(\mathit{Null}, e) \rightarrow \ppure(\mathbb{O}, e)$

$\ppure(T, \PL{u}) \equiv \llbracket \PL{u} \rrbracket \in T' \wedge \Psi(T') = T$

$\ppure(T, \PL{@v}) \equiv \llbracket \PL{this.@v} \rrbracket \in T' \wedge \Psi(T') = T$

$\ppure(\mathbb{O}, \PL{this}) \equiv \mathit{true}$

$\ppure(\mathbb{B}, e_1 == e_2) \equiv \exists T \in \mathcal{T}_{\pure} \bullet \ppure(T, e_1) \wedge \ppure(T,e_2)$

$\ppure(\mathbb{B}, e \PL{ is\_a? C}) \equiv \ppure(\mathbb{O}, e)$

$\ppure(T, e.\PL{m}(\Vector{e})) \equiv \mathit{false}$

$\ppure(T. \PL{new C}(\Vector{e})) \equiv \mathit{false}$

$\ppure(T, \PL{u} := e) \equiv \mathit{false}$

$\ppure(T, \PL{@v} := e) \equiv \mathit{false}$

$\ppure(T, \PL{if } e \PL{ then } s_1 \PL{ else } s_2 \PL{ end}) \equiv \ppure(\mathbb{B},e) \wedge s_i \equiv e_i \wedge \ppure(T, e_i)$ for $i \in \{1,2\}$

$\ppure(T, \PL{while } e \PL{ do } s \PL{ done}) \equiv \mathit{false}$

For every $T \in \mathcal{T}_s$:

$T(o): \mathbb{O} \mapsto T$

$\mathit{safe}_T(o): \mathbb{O} \mapsto \mathbb{B}$

% $T_{init}: T_1 \times ... \times T_n \mapsto \mathit{LExp}( T_1 \times ... \times T_n \mapsto T)$
% 
% For every pure operation $\oplus: {\mathcal{T}_s}^n \mapsto \mathcal{T}_s \in \mathit{op(\Vector{e_{\pure}})}$
% 
% $e_\oplus: T_0 \times ... \times T_n \mapsto \mathit{LExp}( T_0 \times ... \times T_n \mapsto T )$

\underline{Mapping method and constructor calls to logical expressions:}

Note: $l \in \mathit{LExp}$ of type $T$ with free variables $v_0,...,v_n$ of types $T_0, ..., T_n$ can be interpreted
as a function $f_l: T_0  \times ... \times T_n \mapsto T$. We hence denote its type as $LExp(T_0  \times ... \times T_n \mapsto T)$

For every pure operation:
$\Psi(T_0.\PL{m}(T_1,...,T_n) \rightarrow T) = l: LExp(T_0 \times ... \times T_n \mapsto T)$

For every pure constructor:
$\Psi(T_0.\PL{init}(T_1,...,T_n) \rightarrow T) = l: LExp(T_1 \times ... \times T_n \mapsto T)$

\underline{Example for $\mathbb{N}$:}

$\mathbb{N}(o) = \PL{if $o = $ null then 0 else}$

\hspace{2cm} $\PL{if $\llbracket o \rrbracket \not\in \{num\}$ then 0 else}$

\hspace{3cm} $\PL{if $o.\PL{@pred} = null$ then 0 else $\mathbb{N}(o.\PL{@pred}) + 1$ end}$

\hspace{2cm} $\PL{end}$

\hspace{1cm} $\PL{end}$

$\mathit{safe}_{\mathbb{N}}(o) = o \not= null \wedge \llbracket o \rrbracket \in \{num\}$

$\Psi(\mathbb{N}.\PL{init}(\mathit{Null})) = 0$, $\Psi(\mathbb{N}.\PL{init}(\mathbb{N})) = v_1 + 1$,
$\Psi(\mathbb{N}.\PL{add}(\mathbb{N})) = v_0 + v_1$, $\Psi(\mathbb{N}.\PL{succ}()) = v_0 + 1$.

\underline{Translation of pure expressions into logical expressions:}

$\Psi_T(\PL{u}) \equiv T(\PL{u})$

$\Psi_T(\PL{@v}) \equiv T(\PL{this.@v})$

$\Psi_{\mathit{Null}}(\PL{null}) \equiv \PL{null}$

$\Psi_{\mathit{Null}}(e) = p \rightarrow \Psi_{\mathbb{O}}(e) = p$

$\Psi_T(\PL{this}) \equiv T(\PL{this})$

$\Psi_T(e_0.\PL{m}(e_1,...,e_n)) \equiv l[v_0,...,v_n := \Psi_{T_0}(e_0), ..., \Psi_{T_n}(e_n)]$

where $\ppure(T_i, e_i)$ for $i \in \mathbb{N}_n$ and $\Psi(T_0.\PL{m}(T_1,...,T_n) \rightarrow T) = l: LExp(T_0 \times ... \times T_n \mapsto T)$.

$\Psi_T(\PL{new C}(e_1,...,e_n)) \equiv l[v_1,...,v_n := \Psi_{T_1}(e_1), ..., \Psi_{T_n}(e_n)]$

where $\ppure(T_i, e_i)$ for $i \in \mathbb{N}^1_n$ and $\Psi(\Psi(\{C\}).\PL{init}(T_1,...,T_n) \rightarrow T) = l: LExp(T_1 \times ... \times T_n \mapsto T)$.

$\Psi_{\mathbb{B}}(e_1 == e_2) \equiv \Psi_T(e_1) = \Psi_T(e_2)$ where $\ppure(T, e_i)$ for $i \in \{1,2\}$.

$\Psi_{\mathbb{B}}(e \PL{ is\_a? C}) \equiv \llbracket \Psi_{\mathbb{O}}(e) \rrbracket \in \{\PL{C}\}$

$\Psi_T(\PL{if } e \PL{ then } e_1 \PL{ else } e_2 \PL{ end}) \equiv \PL{if } \Psi_{\mathbb{B}}(e) \PL{ then } \Psi_T(e_1) \PL{ else } \Psi_T(e_2) \PL{ end}$



\caption{\label{fig:stat_syntax}Syntax of \textbf{stat}} 
\end{figure}
\todo{extend is\_a? - syntax to allow checking for union types?}

\begin{figure}
 \includegraphics{images/typesystem-dyn.pdf} 
 \includegraphics{images/typesystem-stat.pdf} 
\caption{\label{fig:dyn_stat_typesystem}Type lattices of \textbf{dyn} and \textbf{stat}}
\end{figure}


\subsection{Syntax}

The syntax of both \textbf{dyn} and \textbf{stat} is depicted in Figure~\ref{fig:lang_syntax}.
In \textbf{dyn}, method bodies consist of a statement ($s$) which in contrast to an expression ($e$)
can contain sequential composition.
Expressions are composed of $\PL{null}$, the only constant, local and instance variables (the latter prefixed with
an ``\PL{@}''-sign), the self-reference $\PL{this}$, operators for object identity and dynamic type checks,
method- and constructor calls, assignments, conditionals and while loops. It is important to note that
equality ($\PL{=}$) is desugared to a method call and may hence differ from class to class, while object
identity ($\PL{==}$) is a build-in operation that yields $\mathit{true}$ iff the two expressions refer to
the same object (We stipulate $\PL{null == null}$ yields $\mathit{true}$).

Each class except the predefined class
\textPL{object} must specify a parent class
whose methods are inherited. The inheritance relation must be acyclic. Thus every class transitively inherits
from \textPL{object}. Inherited methods may be overwritten or
renamed (using \textPL{rename}).

Note that it is possible to apply an automatic expansion step adding all inherited methods to each class,
performing the specified renaming and then adding/overwriting the new declarations. We will furthermore
assume this step to be completed and not concern ourselves any further with inheritance or renaming.
This models the situation in actual dynamically typed languages, where inheritance is used as mere code
reuse.

% Each class $C$ has a domain $\mathcal{D}_C$ disjoint from all others and $\Vnull$ is the only element of
% $\mathcal{D}_{Nullclass}$%TODO{is this compatible with our translation?}. The entire value domain of
% type object is thus given by
% $\mathcal{D} = \bigcup_{C \in \Class} \mathcal{D}_C$.
% We use the function $Class: \mathcal{D} \mapsto \Class$ to distinguish values of different classes
% \[Class(v) = C \text{ iff } v \in \mathcal{D}_C.\]

\subsection{Comparing Dyn with Stat}

While extremely similar on the syntactic level, \textbf{dyn} is a pure object-oriented language (objects are the only
values) while \textbf{stat} additionally has basic data types like numbers, booleans and lists (see the type
lattices depicted in Figure~\ref{fig:dyn_stat_typesystem}). However, both provide
the same constants and pure (= side-effect-free) operations on them. Dyn as a theoretical model of 
a dynamically typed OO-language desugares these constants and operations to constructor and method calls
(see Figure~\ref{fig:lang_syntax}),
while \textbf{stat} (like usual in statically typed languages) provides them build-in
($c_{\pure}$ and $\mathit{op}(\Vector{e_{\pure}})$ in Figure~\ref{fig:lang_syntax}).\todo{better references}
While \textbf{dyn} raises type
errors at runtime, \textbf{stat} uses a type inference algorithm to statically ensure the absence of such errors.
This restricts the language, as it also prevents execution of many typesafe programs. We will,
     however, later lift this restriction (see Section~\todo{which one?}).
     
The main syntactic difference between the languages is that \textbf{stat} defines a subset of pure (= side-effect-free)
expressions $e_{\pure}$ and restricts the general side-effecting expressions to have only
pure subexpressions. Note, however, that this very subset can also be identified in \textbf{dyn} using
the $\ppure$-predicate given in Figure~\ref{fig:stat_syntax}.

Also note that this is not a real restriction:
Arbitrary \textbf{dyn}-expressions can be transformed into a sequence of \textbf{stat} statements by
     recursively (and in the order of evaluation) replacing side-effecting subexpressions $e$ by
     local variables $u$ and prepending the assignment $u := e$.
Hoare logic rules for languages with side-effecting expressions (like the ones
     in Section~\ref{sec:HL}) in essence emulate this prepending. While the rules look a bit different,
     this is merely a cosmetic change and causes no problems during verification.

\subsubsection{Semantics}
\label{sec:dyn_semantics}

To facilitate proving soundness using the transformational approach of Apt et al. \cite{AptDeBoerOlderog2012},
we will give our semantics in a style similar to theirs.

A \textbf{dyn} program consists of a main statement $S$ and a set of classes $\Class$, each with its set of method
declarations $\Method_C \subseteq \Method$ and instance variables $\Var_C \subseteq \Var_I$ for $C \in \Class$.
$\Var_C$ includes all instance variables used in methods of $C$.

We denote the set of all methods as $\Method$ and the set of all variables as $\Var = \Var_L \uplus \Var_I$
where $\Var_L$ and $\Var_I$ are the
sets of local- and instance variables respectively. $\Var_S = \{this, \result\} \subset \Var_L$ is a set of
special variables.
The self-reference $this$ always references the current object and is not allowed to be assigned
to in programs, $\result$ holds the result of expressions and
statements after their execution and is not allowed to be used in programs.

As a pure object-oriented languages, objects are the only values in \textbf{dyn}.
The value domain $\Domain$ thus is the set of all objects. States, ranged
over by $\sigma, \tau$ are
overloaded to mean both
a mapping from simple variables to values (usually called an environment) as well as
a mapping from objects to their local states (usually called a heap).
%
\begin{definition} \textbf{(State)}
\begin{itemize}
 \item \emph{Local states} are partial functions in $\Sigma_L = \Var_I \partialmapsto \Domain$
 mapping instance variables to their referenced objects.
 \item \emph{Environments} are partial functions in $\Sigma_E = \Var_L \partialmapsto \Domain$
 mapping local variables to their referenced objects and
 \item \emph{Heaps} are functions in $\Sigma_H = \Domain \mapsto \Sigma_L$
 mapping objects to their local states.
 \item \emph{Proper States} are tuples of environments and heaps in $\Sigma = \Sigma_E \times \Sigma_H$. For all
proper states $\sigma = (\sigma_E, \sigma_H) \in \Sigma$ we will use the notation $\sigma(x)$ to denote
the function
\[\sigma(x) = \begin{cases}
                            \sigma_E(x) & \text{if } x \in \Var_L \\
                            \sigma_H(\sigma_E(this))(x) & \text{if } x \in \Var_I \\
                            \sigma_H(x) & \text{if } x \in \Domain
                          \end{cases}\]
                          
where $this$ is a special variable always referencing the current object. We extend this notation to
sequences of dereferences and write $\sigma(x.@v)$ instead of $\sigma(\sigma(x))(@v)$ for $x \in \Var_L$
or $\sigma(x)(@v)$ for $x \in \Domain$.
 \item \emph{States} are either proper states, $\mathbf{fail}$ or $\mathbf{typeerror}$.
\end{itemize}
\end{definition}
%
\begin{definition} \textbf{(State Update)}\newline
 For any (possibly partial) function $f: A \mapsto B$, $a,a' \in A$ and $b \in B$ a \emph{function update} is defined as

 \[f[a := b](a') = \begin{cases}
   b & \text{if } a = a' \\
   f(a') & \text{otherwise.}
 \end{cases}\]

\noindent For any proper state $\sigma = (\sigma_E, \sigma_H) \in \Sigma$ a \emph{state update} is defined as
 
 \[\sigma[x := v] = \begin{cases}
                    (\sigma_E[x := v], \sigma_H) & \text{if } x \in \Var_L \\
                    (\sigma_E, \sigma_H[o := \sigma_L[x := v]]) & \text{if } x \in \Var_I \\
                    (\sigma_E, \sigma_H[x := v]) & \text{if } x \in \Domain
                   \end{cases}\]
                   
 where $o = \sigma_E(this)$ and $\sigma_L = \sigma_H(o)$.
\end{definition}
%
To keep track of instance-class relationships we use
class references and introduce
a distinct object $\oC_C$ of class $\mathit{object}$ for every class $C$ as
well as
a special instance variable $@\mathbf{c}$ that is defined ($@\mathbf{c} \in dom(\sigma(o))$) iff the
object $o$ is active and references $\oC_C$ ($\sigma(o.@\mathbf{c}) = \oC_C$) iff the object $o$ is an
instance of class $C$. We do not allow $@\mathbf{c}$ to be used in programs.

Thus $\sigma(\oC_C.@\mathbf{c}) = \oC_{\mathit{object}}$ for all classes $C$ and
proper states $\sigma$.
Furthermore, we model object creation as object activation and introduce
an infinite sequence of objects $o_1,o_2,...$ that are initially inactive and do not yet have
any instance variables as well as 
a function $\creation: \Sigma \mapsto \mathcal{D}$ mapping a proper state $\sigma$ to the object $o_i$
with the least index $i$ that is inactive in $\sigma$.

Each class $C$ then has an initial local state $\mathit{init}_C \in \Sigma_L$ with
$\mathit{init}_C(@\mathbf{c}) = \oC_C$ and $\mathit{init}_C(@v) = \Vnull$ for all $@v \in V_C$ that
is used in the rule for object creation.

%
% \begin{itemize}
%  \item an infinite sequence of objects $o_1,o_2,...$ that are initially inactive and do not yet have
%        any instance variables.
%  \item a function $\creation: \Sigma \mapsto \mathcal{D}$ mapping a proper state $\sigma$ to the object $o_i$
%        with the least index $i$ that is inactive in $\sigma$.
%  \item For each class $C$, an initial local state $\mathit{init}_C \in \Sigma_L$ with
%        $\mathit{init}_C(@\mathbf{c}) = \oC_C$ and $\mathit{init}_C(@v) = \Vnull$ for all $@v \in V_C$.
% \end{itemize}
%
%
%
% Statements and expressions in \textbf{dyn} all have a return value, represented semantically by the 
% special variable $\result \in V_S$, that may not be used in \textbf{dyn} programs.
% 
We define predicates for testing for instances of class $\mathit{bool}$ (representing boolean values).
The truth value is encoded by setting the instance variable $@\mathrm{to\_ref}$
to $\Vnull$ or $\not= \Vnull$.
%
\begin{align*}
\mathit{bool}(\sigma, v) \equiv & \sigma(v) \not= \Vnull \wedge \sigma(v.@\mathbf{c}) = \oC_{bool} \\
\mathit{bool}(\sigma, v, b) \equiv & \mathit{bool}(\sigma,v) \wedge b \leftrightarrow \sigma(v.@\mathrm{to\_ref}) \not= \Vnull 
\end{align*}
%
The block-construct
``begin local $\Vector{u} := \Vector{v}; S$ end`` is used to maintain a stack discipline. Both the block
and the parallel assignment are not part of \textbf{dyn}'s syntax but only used in its semantics to conceptually
split the otherwise unwieldy method call rule.
%
\ifx \version\extended
  The structural operational semantics of \textbf{dyn} is then given in Figure~\ref{fig:dyn_op_sem}.
  There, the empty \textbf{dyn} program is represented by $\emptyP$ and we define $\emptyP; S \equiv S$.
\else
  Selected rules from the structural operational semantics of \textbf{dyn} are given in Figure~\ref{fig:dyn_op_sem},
  the complete semantics is available in \cite{extended}.
  In the rules the empty \textbf{dyn} program is represented by $\emptyP$ and we define $\emptyP; S \equiv S$.
\fi
%
\begin{figure}
\begin{enumerate}
\ifx \version\extended
 \item $\langle \Vnull, \sigma\rangle  \step \langle\emptyP, \sigma[\result := \Vnull]\rangle $

 \item $\langle v, \sigma\rangle  \step \langle\emptyP, \sigma[\result := \sigma(v)]\rangle $ where $v \in \Var$
\fi

 \item \AxiomC{$\langle E, \sigma\rangle  \mstep \langle\emptyP, \tau\rangle $}
       \RightLabel{where $v \in V$}
       \UnaryInfC{$\langle v := E, \sigma\rangle  \step \langle\emptyP, \tau[v := \tau(\result)]\rangle $}
       \DisplayProof
 
\ifx \version\extended
 \item \AxiomC{$\langle S_1, \sigma\rangle  \step \langle S_2, \tau\rangle $}
       \UnaryInfC{$\langle S_1; S, \sigma\rangle  \step \langle S_2; S, \tau\rangle $}
       \DisplayProof
\fi

 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle\emptyP, \tau\rangle $}
       \AxiomC{$\mathit{bool}(\tau, \result, \mathrm{true})$}
       \BinaryInfC{$\langle \PL{if } B \PL{ then } S_1 \PL{ else } S_2 \PL{ end}, \sigma\rangle  \step \langle S_1, \tau\rangle $}
       \DisplayProof

 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle\emptyP, \tau\rangle $}
       \AxiomC{$\mathit{bool}(\tau, \result, \mathrm{false})$}
       \BinaryInfC{$\langle \PL{if } B \PL{ then } S_1 \PL{ else } S_2 \PL{ end}, \sigma\rangle  \step \langle S_2, \tau\rangle $}
       \DisplayProof

 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle\emptyP, \tau\rangle $}
       \AxiomC{$\tau(\result) = \Vnull$}
       \BinaryInfC{$\langle \PL{if } B \PL{ then } S_1 \PL{ else } S_2 \PL{ end}, \sigma\rangle  \step \langle \emptyP, \mathbf{fail}\rangle $}
       \DisplayProof

 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle\emptyP, \tau\rangle $}
       \AxiomC{$\neg \mathit{bool}(\tau, \result)$}
       \BinaryInfC{$\langle \PL{if } B \PL{ then } S_1 \PL{ else } S_2 \PL{ end}, \sigma\rangle  \step \langle \emptyP, \mathbf{typeerror}\rangle $}
       \DisplayProof

\ifx \version\extended
 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle\emptyP, \tau\rangle $}
       \AxiomC{$\mathit{bool}(\tau, \result, \mathrm{true})$}
       \BinaryInfC{$\langle \PL{while } B \PL{ do } S \PL{ done}, \sigma\rangle  \step \langle S; \PL{while } B \PL{ do } S \PL{ done}, \tau\rangle $}
       \DisplayProof
 
 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle \emptyP, \tau\rangle $}
       \AxiomC{$\mathit{bool}(\tau, \result, \mathrm{false})$}
       \BinaryInfC{$\langle\PL{while } B \PL{ do } S \PL{ done}, \sigma\rangle  \step \langle \Vnull, \tau\rangle $}
       \DisplayProof

 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle \emptyP, \tau\rangle $}
       \AxiomC{$\tau(\result) = \Vnull$}
       \BinaryInfC{$\langle\PL{while } B \PL{ do } S \PL{ done}, \sigma\rangle  \step \langle \emptyP, \mathbf{fail}\rangle $}
       \DisplayProof

 \item \AxiomC{$\langle B, \sigma\rangle  \mstep \langle \emptyP, \tau\rangle $}
       \AxiomC{$\neg\mathit{bool}(\tau,\result)$}
       \BinaryInfC{$\langle\PL{while } B \PL{ do } S \PL{ done}, \sigma\rangle  \step \langle \emptyP, \mathbf{typeerror}\rangle $}
       \DisplayProof
\fi
 \item $\langle\Vector{l} := \Vector{l'}, \sigma\rangle  \step \langle\emptyP, \sigma[\Vector{l} := \sigma(\Vector{l'})]\rangle $ where $\Vector{l}, \Vector{l'} \in \Var^+_L$

 \item $\langle\PL{begin local } \Vector{u} := \Vector{v}; S \PL{ end}, \sigma\rangle  \step \langle\Vector{u} \Vector{\overline{u}} := \Vector{v} \Vector{\Vnull}; S; \Vector{u} \Vector{\overline{u}} := \sigma(\Vector{u}\Vector{\overline{u}}), \sigma\rangle$

 where $\{\Vector{\overline{u}}\} = \Var_L \setminus (\{\Vector{u}\} \cup \Var_S)$ and $\Vector{\Vnull}$ is a fitting sequence of $\Vnull$ values.

 \item \AxiomC{$\langle E_i, \sigma_i\rangle \mstep \langle \emptyP, \sigma_{i+1}\rangle $ for all $i \in \mathbb{N}_n$}
       \UnaryInfC{$\langle E_0.m(E_1,...,E_n), \sigma_0\rangle  \step \langle\PL{begin local } this, \Vector{u} := \sigma_1(\result),...,\sigma_{n+1}(\result); S \PL{ end}, \sigma_{n+1}\rangle$}
       \DisplayProof
       
 where $\sigma_1(\result) \not= \Vnull$, $\PL{method } m(u_1,...,u_n) \{ S \} \in \Method_C$ and $\sigma_1(\result.@\mathbf{c}) = \oC_C$.
 
 \item \AxiomC{$\langle E_0, \sigma_0\rangle  \mstep \langle\emptyP, \sigma_1\rangle $}
       \AxiomC{$\sigma_1(\result) = \Vnull$}
       \BinaryInfC{$\langle E_0.m(E_1,...,E_n), \sigma_0\rangle  \step \langle\emptyP, \mathbf{fail}\rangle $}
       \DisplayProof
 
 \item \AxiomC{$\langle E_0, \sigma_0\rangle  \mstep \langle\emptyP, \sigma_1\rangle $}
       \AxiomC{$\sigma_1(\result) \not= \Vnull$}
       \BinaryInfC{$\langle E_0.m(E_1,...,E_n), \sigma_0\rangle  \step \langle\emptyP, \mathbf{typeerror}\rangle $}
       \DisplayProof

 where $\PL{method } m(u_1,...,u_n) \{ S \} \not\in \Method_C$ and $\sigma_1(\result.@\mathbf{c}) = \oC_C$ % {Class(\sigma_1(\result))}$
       
 \item $\langle\PL{new } C(E_1,...,E_n), \sigma\rangle  \step \langle\mathbf{new}_C.init(E_1,...,E_n), \sigma\rangle $

 \item $\langle\mathbf{new}_C, \sigma\rangle  \step \langle\emptyP, \sigma[o := \mathit{init}_C][\result := o]\rangle $ where $o = \creation(\sigma)$

\end{enumerate}
\caption{\label{fig:dyn_op_sem} \ifx \version\conference Excerpt from \textbf{dyn}'s structural operational semantics \else Dyn's structural operational semantics \fi}
\end{figure}
%
Note that the rule for assignments is able to handle side-effecting expressions and the rules
for conditionals and method calls have distinguished behaviors for failures and type errors
in case of unsuitable conditions/receivers. 
The reason for this distinction of failures and type errors
is that type systems are traditionally only concerned with the latter.
The rules for while loops were omitted as they merely
mirror the behavior of conditionals.

The rules for method calls (or more precisely: $begin local$-blocks)
and object creation ensure proper instantiation of local / instance
variables by automatically initializing them to $\Vnull$. 
We hence do not need to consider the case of uninitialized variables as discussed at the beginning of
Section~\ref{sec:language}.

Note also the handling of special variables in method calls: $\this$ is set to the receiver of the
method call while $\result$ intentionally remains unmodified to pass the return value back to the caller.

Constructors are normal methods conventionally named $\mathit{init}$ that are called on newly created
instances
directly after they were created. The instance creation (activation) itself is called $\textbf{new}_C$.
Note that new $C(...)$ returns the constructor's return value
which is not necessarily the newly created instance. Also note that calling new $C'(...)$ for a class $C'$
that does not have a method $init$ results in a $\mathbf{typeerror}$.


==> sections/proof_rec_to_quant.tex <==
\begin{theorem}[Translating Recursion]\label{thm:rec_to_quant}
 Assuming that the assertion language $\mathcal{A}$ contains weak second-order quantification, then
 for any (bounded) recursive predicate $p(a_1,...,a_n)$ defined in $\mathcal{A}$, there exists a
 non-recursive predicate $p'(a_1,...,a_n)$ using second-order quantification such that
 \[\forall a_1,...,a_n \bullet p'(a_1,...,a_n) \leftrightarrow p(a_1,...,a_n)\].
\end{theorem}

\begin{proof}
 By Lemma~\ref{lem:mutual_rec} any mutually recursive predicates can be transformed into one tree-recursive one.
 By Lemma~\ref{lem:tree_rec}, and the assumption that the recursion-depth is bounded, the tree-recursive
 predicate can be transformed into one using weak second-order quantification.\qed
\end{proof}

\begin{lemma} [Linear Recursion]
 Assuming that the assertion language $\mathcal{A}$ contains weak second-order quantification, then
 for any (bounded) linear recursive predicate $p(a_1,...,a_n)$ defined in $\mathcal{A}$, there exists a
 non-recursive predicate $p'(a_1,...,a_n)$ using second-order quantification such that
 \[\forall a_1,...,a_n \bullet p'(a_1,...,a_n) \leftrightarrow p(a_1,...,a_n)\].
\end{lemma}

\todo{proof}

\begin{lemma} [Tree Recursion]\label{lem:tree_rec}
 Assuming that the assertion language $\mathcal{A}$ contains weak second-order quantification, then
 for any (bounded) tree recursive predicate $p(a_1,...,a_n)$ defined in $\mathcal{A}$, there exists a
 non-recursive predicate $p'(a_1,...,a_n)$ using second-order quantification such that
 \[\forall a_1,...,a_n \bullet p'(a_1,...,a_n) \leftrightarrow p(a_1,...,a_n)\].
\end{lemma}
 
\todo{proof}

\begin{lemma} [Mutual Recursion]\label{lem:mutual_rec}
 For any (finite) set of mutually recursive predicates $p_1(a_{1,1},...,a_{1,n_1}), ..., p_k(a_{k,1},...,a_{k,n_k})$
 there exists a tree recursive predicate $p(a_1,...,a_{n_1})$ such that
 \[\forall a_1,...,a_{n_1} \bullet p_1(a_1,...,a_{n_1}) \leftrightarrow p(a_1,...,a_{n_1})\].
\end{lemma}
Note that without loss of generality we assume the first predicate in the set to be the main point of entry. By
reordering the predicates the Theorem may be applied to any other choice as well.

\begin{proof}
 By induction on the size of the recursive cycle.
 \textbf{Induction Basis:} A single predicate can only call itself. Hence the worst possible case is tree recursion.
 \textbf{Induction Hypothesis:} Assume above lemma applies to all recursive cycles of size up to $n$.
 \textbf{Induction Step:} Given a recursive cycle of size $n+1$ (any predicate $p_i$ invokes $p_{i+1}$ and
 $p_{n+1}$ invokes $p_1$ again), one can construct an equivalent recursive cycle of size $n$ by inlining
 the body of the predicate $p_i$ (for some $i$) into its predecessor $p_{i-1}$ and properly substituting
 its arguments for those used in the invokation. By the Induction Hypothesis, there hence exists an
 equivalent tree recursive predicate.\qed
\end{proof}




==> sections/reducing.tex <==
Our methodology targets languages like JavaScript, Python and Ruby, that are both object-oriented
and dynamically typed. Such languages hence do not use a static type system to ensure
that operations are performed on suitable operands. Instead of rejecting programs deemed unsafe at
compile time, they allow
every syntactically correct program to be executed and raise type errors at runtime when
\begin{itemize}
 \item a method call is not supported by its receiver (in this arity),
 \item the condition of a conditional or while loop does not evaluate to a boolean value or
 \item a variable is accessed that has not been previously assigned
\end{itemize}
While ``message not understood''-errors are fundamentally linked to type-checking in
OO-languages differentiating multiple object types, conditionals in dynamically typed
languages often accept arbitrary conditions. However, the second error condition
represents a common error class occuring when a built-in operation only supports a
fixed set of input types. Omitting it would cause no problems.

Although optional variables are common in practice, the third point will be left as future work.
We will consider all local variables used in a method to
be initialized to $\Vnull$ at the beginning of each execution and all instance variables
of a class to be initialized to $\Vnull$ when creating an instance of this class.

Also, many dynamically typed languages treat type errors as exceptions, allowing them to be
caught and handled. For simplicity
we will not introduce exceptions into our model languages and consider type errors as fatal.


==> sections/trans_programs.tex <==
For our transformation, direct access to return values will be neccessary. We therefore introduce
a normal global variable $r$ that is not used in the dyn program to be transformed but may be
accessed like any other variable in the resulting simple oo-program.
The transformation will ensure that after executing a resulting oo-statement, $r = \mathbf{r}$.

%- introduce predicate C: object -> boolean
%                     true   if \sigma(s) \in D_C
%     \sigma(C(s)) =  false  otherwise

% - map classes with their sets of methods to a global set of method declarations
%    m@C(u_1,...,u_n) :: S

% map the statement s.m(t_1,...,t_n) to S_n which is inductively defined as follows
% - S_0 \equiv fail()
% - S_{i+1} \equiv if C_{i+1}(s) then s.m@C_{i+1}(t_1,...,t_n) else S_i fi
% where {C_1,...,C_n} = { C \in Classes | C supports method m with n arguments }
% and fail() \equiv if false -> skip fi

% mapping: constructor -> new + call to init method

Like dyn, simple object-oriented programs use two disjoint sets of variable names, $Var$ and $IVar$.
However, local variables and instance variables are only distinguished by requiring $Var \cap IVar = \emptyset$
\cite[page 7]{AptDeBoerOlderog2012} and not syntactically, like in dyn. By simply choosing all the names in
$IVar$ to begin with an $@$-sign, we remove the neccessity of a mapping between variable names.

% dyn
% - hierarchy of classes, each with a set of methods
% - instance variables of a class are those assigned in its constructor, init
% - disjoint domains D_C for every class C
% - null is only element \in D_{NullClass}
% oo
% - no classes
% - set of methods (can be called on every object)
% - set of instance variables (for all objects)
% - introduce: predicate C(l) for each class C: \sigma \models C(l) iff \sigma(l) \in D_C
%   - give each class C a unique integer constant N_C
%   - introduce an unused integer instance variable $\mathbf{c}$
%   - set $\mathbf{c}$ to N_C whenever an object is created by new_C
%   - define C(l) as l.\mathbf{c} = N_C

In dyn-programs, there is a hierarchy of classes each with its set of methods.
%The classes have disjoint domains ($\mathcal{D}_C = \{ o \in \mathcal{D} | o.@\mathbf{c} = o_C \}$ for each class $C$) populated by their respective instances.
The null value is the only instance of class $\mathbf{Nullclass}$.
A classes instance variables are those assigned in its constructor.\todo{reference to a more detailed explanation}

On the contrary, simple object-oriented programs as defined in \cite{AptDeBoerOlderog2012} do neither
support any classes nor distinguish any values of type object. There is only a global set of methods $D$
which can be called on any object. Also, the full set $IVar$ of instance variables can be accessed on
any object.

To properly model the behaviour of dyn programs with respect to classes, we add a previously unused
instance variable $\mathbf{c}$ of type integer to our simple oo-programs, assign each class $C$ in
our dyn program
a unique integer constant $N_C \in \mathbb{N}$ and initialize $\mathbf{c}$ to $N_C$ whenever an object
of class $C$ is created with $\mathbf{new}$.

We now define a function $\Theta: \Sigma_{dyn} \mapsto \Sigma_{oo}$ mapping dyn-states $\sigma$ into
states of simple object-oriented programs $\Theta(\sigma)$.

% mapping states:
% - transforming the object-based o_C's into N_C's
% - making the partial functions total
% - mapping the objects from $\mathcal{D}$ to $\mathcal{D}_{oo}$

\begin{itemize}
 \item $\Theta(\mathbf{fail}) = \mathbf{fail}$
 \item $\Theta(\mathbf{typeerror}) = \mathbf{typeerror}$
 \item $\Theta(\sigma) = \sigma'$
 
 where $\sigma' = (\sigma'_E, \sigma'_H) \in \Sigma_{oo}$ can be derived from the state $\sigma = (\sigma_E, \sigma_H) \in \Sigma_{dyn}$ as follows
 
 \begin{itemize}
  \item mapping all dyn-objects $o \in \mathcal{D}$ to oo-objects $\Theta(o) \in \mathcal{D}_{\mathbf{object}}$.
  \item deriving a total environment $\sigma'_E$ from the partial $\sigma_E$ by assigning $null$ to all variables $v \in Var \setminus dom(\sigma_E)$.
  \item making all local states $\sigma_H(o)$ total by assigning $null$ to each instance variable $@v \in IVar \setminus dom(\sigma_H(o))$.
  \item for all active objects $o$, substituting the instance variable $@\mathbf{c}$ with $\sigma(o)(@\mathbf{c}) = o_C$ by
  an instance variable $\mathbf{c}$ of type int such that $\sigma'(\Theta(o))(\mathbf{c}) = N_C$.
  \item add a simple variable $r$ of type $\mathbf{object}$ and a sequence of simle variables $l_1,l_2,...$
  of type $\mathbf{object}$ that can be used by
  the transformation as fresh variables. Map all these variables to $null$.
 \end{itemize}
\end{itemize}

Next, we extend the mapping $\Theta$ to map statements of dyn-programs to statements of simple OO-programs:

%---NEW----

\begin{itemize}
 \item $\Theta(S_1; S_2) \equiv \Theta(S_1); \Theta(S_2)$
 \item $\Theta(null) \equiv r := null$
 \item $\Theta(x) \equiv r := x$
 \item $\Theta(@x) \equiv r := @x$
 \item $\Theta(this) \equiv r := this$
 \item $\Theta(l := E) \equiv \Theta(E); l := r$
 \item $\Theta(@v := E) \equiv \Theta(E); @v := r$
 \item $\Theta(E_0.m(E_1,...,E_n)) \equiv$\newline
 \hspace*{0.5cm}$\Theta(E_0); l_0 := r; ...; \Theta(E_n); l_n := r;$ if $l_0 \not= null$ then $S_k$ else $\mathbf{fail}$ fi\newline
 where $l_i$ are fresh for all $i \in \{0,...,n\}$ and
 $S_k$ is defined inductively as follows
 \begin{itemize}
  \item $S_0 = \textbf{typeerror}$
  \item $S_i =$ if $l_0.\mathbf{c} = N_{C_i}$ then $l_0.m@C_i(l_1,...,l_n, \overline{null})$ else $S_{i-1}$ fi
 \end{itemize}
 where $\{C_1,...,C_k\}$ is the set of classes supporting a method $m$ of arity $n$ and $\overline{null}$ is a
 sequence of $|Var|-n$ $null$-constants.
 \item $\Theta($new $C(E_1,...,E_n)) \equiv$\newline
 \hspace*{0.5cm} $\Theta(E_1); l_1 := r; ...; \Theta(E_n); l_n := r; r := \mathbf{new}; r.\mathbf{c} := N_C; r.init(l_1,...,l_n)$\newline
 \hspace*{1cm} where $l_i$ are fresh for all $i \in \{1,...,n\}$
 \item $\Theta($if $E$ then $S_1$ else $S_2$ end$) \equiv$\newline
 \hspace*{0.5cm}$\Theta(E); r.to\_ref();$ if $r \not= null$ then $\Theta(S_1)$ else $\Theta(S_2)$ fi
 \item $\Theta($while $E$ do $S$ done$) \equiv$\newline
 \hspace*{0.5cm}$\Theta(E); r.to\_ref();$ while $r \not= null$ do $\Theta(S); \Theta(E); r.to\_ref()$ od; r := null
 \item $\Theta(\overline{l} := \overline{l'}) \equiv \overline{l} := \overline{l'}$
 \item $\Theta($begin local $\overline{u} := \overline{l}; S$ end$) \equiv $begin local $\overline{u} := \overline{l}; \Theta(S)$ end
\end{itemize}


%---END NEW----


% $\Theta(null) \equiv null$
% 
% $\Theta(x) \equiv x$ for every local variable $x$.
% 
% $\Theta(@x) \equiv @x$, $@x$ on the left-hand-side denoting an OO-instance variable and on the right-hand-
% side a dyn-instance variable.
% 
% $\Theta(this) = this$
% 
% This mapping satisfies the following properties
% 
% \begin{lemma}
% For all proper states $\sigma$ the following hold.
% \begin{itemize}
%  \item For all expressions $s$, \[\sigma(s) = \Theta(\sigma)(\Theta(s)).\]
%  \item For all instance variables @u and objects d
%  \[\Theta(\sigma[@u := d]) = \Theta(\sigma)[\Theta(@u) := d].\]
% \end{itemize} 
% \end{lemma}



% Now, we can extend the mapping to restricted dyn-statements:
% 
% \begin{definition} \textbf{(Translation)} $\Theta: S_{rdyn} \mapsto S_{oo}$ is defined inductively over the structure of
% restricted dyn statements.
% 
% \begin{itemize}
%  \item $\Theta(S_1;S_2) \equiv \Theta(S_1); \Theta(S_2)$
%  \item $\Theta(r := E) \equiv r := \Theta(E)$
%  \item $\Theta(l := r) \equiv l := r$
%  \item $\Theta(@v := r) \equiv @v := r$
% % \item $\Theta(r := l_0.m(l_1,...,l_n)) \equiv l_0.m(l_1,...,l_n)$ \todo{old}
%  \item $\Theta(r := l_0.m(l_1,...,l_n)) \equiv$ if $l_0 \not= null$ then $S_n$ else $\mathbf{fail}$ end
% 
%  where $S_n$ is defined inductively as follows
%  \begin{itemize}
%   \item $S_0 = \textbf{typeerror}$
%   \item $S_i =$ if $l_0.\mathbf{c} = N_{C_i}$ then $l_0.m@C_i(l_1,...,l_n)$ else $S_{i-1}$ fi
%  \end{itemize}
%  where $\{C_1,...,C_n\}$ is the set of classes supporting a method $m$ of arity $n$.
%  
%  \item $\Theta(r := $ new $C(l_1,...,l_n)) \equiv r := \mathbf{new}; r.\mathbf{c} := N_C; r.init(l_1,...,l_n)$
%  \item $\Theta(r := $ if $l$ then $S_1$ else $S_2$ end$) \equiv$\newline
%  \hspace*{1cm} $l.to\_ref();$ if $r \not= null$ then $\Theta(S_1)$ else $\Theta(S_2)$ fi
%  \item $\Theta(r :=$ while $l$ do $S$ done$) \equiv$\newline
%  \hspace*{1cm} $l.to\_ref();$ while $r \not= null$ do $\Theta(S); l.to\_ref()$ od$; r := null$
%  \item $\Theta(\overline{l} := \overline{l'}) \equiv \overline{l} := \overline{l'}$
%  \item $\Theta($begin local $\overline{u} := \overline{l}; S$ end$) \equiv $begin local $\overline{u} := \overline{l}; \Theta(S)$ end
% \end{itemize}
% \end{definition}

Finally, we transform every method declaration in the restricted dyn-program

\[ method(u_1,...,u_n) \{ S \} \in C \]

into a method declaration in the simple OO-proram

\[ m@C(u_1,...,u_n, \overline{l_i}) :: \Theta(S) \]

where $\{\overline{l_i}\} = Var_{dyn} \setminus \{u_i\}$.

Note that any such method will automatically store its return value in $r$ since its body is a converted
dyn statement. Since $r$ is a global variable and cannot be overwritten by
method arguments or local variables, methods will always terminate with their result stored in $r$.
The same holds true for the branches of an if-statement. Thus neiter the method calls nor if-statements must
explicitly store the result in $r$.

\subsection{correctness of the transformation}

\begin{lemma} \label{transformation_lemma_for_Theta} \textbf{(Transformation)} For all
dyn-programs $S$, all sets of classes $\mathcal{C}$ with method declarations $M_C$, all proper states
$\sigma$, and all proper or $\mathbf{fail}$ or $\mathbf{typeerror}$ states $\tau$,
\[ <S,\sigma> \mstep <\mathbf{e},\tau>\text{ iff }<\Theta(S),\Theta(\sigma)> \mstep <E,\Theta(\tau)> \]
\end{lemma}

\todo{proof}
%2do:
% S ::= r := new C(l_1,...,l_n)
%ok:
% E ::= null, x, @x, this
% S ::= S;S, r := E, l := r, @v := r, r := l_0.m(l_1,...,l_n), if, while
Finally, the following theorem establishes correctness of $\Theta$ as a homomorphism. For this theorem
we extend $\Theta$ to sets of states in the obvious way.

\begin{theorem}
\label{correctness_of_Theta}
 \textbf{(Correctness of $\Theta$)} For all dyn-programs $S$, all sets of classes $\mathcal{C}$ with
 method declarations $M_C$, and all proper states $\sigma$ the following holds:

\begin{itemize}
 \item $ \Theta(\mathcal{M}\llbracket S \rrbracket(\sigma)) = \mathcal{M}\llbracket \Theta(S) \rrbracket(\Theta(\sigma))$
\end{itemize}

where $S$ is considered in the context of the set $\mathcal{C}$ or dyn class declarations (each with its
corresponding method declarations $M_C$) and the corresponding simple object-oriented program $\Theta(S)$ in
the context of the set of method declarations $\Theta(\mathcal{C})$.
\end{theorem}

\textbf{Proof.} Theorem~\ref{correctness_of_Theta} is a direct consequence of Lemma~\ref{transformation_lemma_for_Theta}.


% \subsection{correctness of restriction}
% \todo{merge with previous section}
% % $\Gamma(\sigma) = \sigma[r := \mathbf{r}]$  (should never overwrite anything as $r$ is not used in the
% % program to be transformed)
% 
% Let $l_1,l_2,...$ be a sequence of variables that are not used anywhere in the program to be restricted and
% used by the $\Gamma$-translation whenever a fresh variable is needed.
% 
% We use $\check{\sigma}$ to denote the state $\sigma$ with all mappings to $r, l_1, l_2,...$ removed.
% 
% \begin{lemma}
% \label{transformation_lemma_for_Gamma}
% $\forall S,\sigma,\tau$
% 
% $\bullet <S, \check{\sigma}> \mstep <\mathbf{e},\check{\tau}>$ iff $<\Gamma(S), \sigma> \mstep <\mathbf{e},\tau>$
% \end{lemma}
% 
% \textbf{Proof.} By induction over the structure of dyn statements.
% %ok: null,v,@v,this, s;s, v := E, @v := E, e.m(e1,...,en),new C(e1,...,en), if, while
% 
% The only interesting case being Sequential Composition: $\Gamma(S_2)$ is executed in some state $\Gamma(\tau)$ instead of $\tau$, which
% is identical top $tau$ except for the added variable $r$. Therefore, if the first statement of $\Gamma(S_2)$
% would be of the form $l := r$, its behaviour could differ from when it is executed in state $\tau$. However,
% $\Gamma(S_2)$ is a translated dyn program and the $\Gamma$-translation will never yield a program beginning
% with $l := r$.
% 
% 
% \begin{theorem}
% $\forall S,\sigma$
% 
% $\bullet \Gamma(\mathcal{M}\llbracket S \rrbracket(\sigma)) = \mathcal{M}\llbracket \Gamma(S) \rrbracket(\Gamma(\sigma))$
% \end{theorem}
% 
% \textbf{Proof.} direct consequence of Lemma~\ref{transformation_lemma_for_Gamma}



\subsection{Soundness}

\todo{proof soundness and completeness}

\todo{translate assertions of dyn-programs to assertions of oo-programs}

We extend $\Theta$ to assertions:

$\Theta(p) = p$

\begin{lemma} \textbf{(Assertion)}
\label{assertion_lemma}
 For all assertions $p$ and all proper states $\sigma$
 \[ \sigma \models p \text{ iff } \Theta(\sigma) \models \Theta(p). \]
\end{lemma}

\textbf{Proof.} straightforward

\begin{corollary} \textbf{(Translation I)}
 For all correctness formulars $\{p\} S \{q\}$ where S is a dyn-program,
 \[ \models \{p\} S \{q\} \text{ iff } \models \{\Theta(p)\} \Theta(S) \{\Theta(q)\} \]
and
 \[ \models_{sp} \{p\} S \{q\} \text{ iff } \models_{sp} \{\Theta(p)\} \Theta(S) \{\Theta(q)\} \]
\end{corollary}

\textbf{Proof.} Follows directly from the Assertion Lemma~\ref{assertion_lemma} and the correctness of
$\Theta$ (Theorem~\ref{correctness_of_Theta}).

\todo{translate proofs of dyn-programs to assertions of oo-programs}

\subsection{Completeness}



==> sections/type_inference_and_type_safety.tex <==
\todo{use another symbol for typings ($s$ is for statements)}
\newcommand{\Fabstract}{\alpha}
\newcommand{\Fconcrete}{\gamma}
\newcommand{\smin}{s^{\dagger}}

In this paper, we regard a \emph{type error} as a fatal runtime event occurring when a method is called
on a receiver that does not support it (message not understood) or when the condition of a
conditional or while loop does not evaluate to a boolean value.

A program $\pi$ is called \emph{typesafe} when no execution of $\pi$ can possibly result in a type error.
\emph{Type safety} is the problem of deciding whether a given program is typesafe. Since type errors
can be regarded as a form of output, type safety is a semantic property and hence undecidable for
Turing complete languages by Rice's theorem.\todo{check the exact formulation}


A \emph{type} $t$ is an element of a complete lattice $(\mathcal{T}, \sqsubseteq)$. \emph{Type abstraction}
means to abstract from the infinite domain of values $\mathcal{D}$ to the finite domain of types
$\mathcal{T}$ using a Galois
connection (a pair of a monotone abstraction function $\Fabstract: 2^\mathcal{D} \mapsto \mathcal{T}$ and a
monotone concretization function $\Fconcrete: \mathcal{T} \mapsto 2^\mathcal{D}$, such that
$\Fabstract \circ \Fconcrete \sqsubseteq id_{\mathcal{T}}$ and
$\Fconcrete \circ \Fabstract \sqsubseteq id_{\mathcal{D}}$).

A \emph{typing} $s$ of a program $\pi$ is a function mapping elements of a domain $x \in dom(s)$ to a
type $s(x) \in \mathcal{T}$. Matching the definition of a type error, it is required that for
all method calls $e_0.\PL{m}(\Vector{e})$ in $\pi$,
$e_0 \in dom(s)$ and for every conditional or while loop with a condition $e$ in $\pi$, $e \in dom(s)$.
A typing whose domain contains no further elements is called \emph{minimal}.
It is important to stress that a subexpression occurring multiple times in $\pi$ is treated as
multiple different expressions. One can think of expressions as represented by their parse tree node.

A typing $s$ for a program $\pi$ is called \emph{safe} if in every execution of $\pi$, every subexpression $e \in dom(s)$ is
evaluated to a value of type $t \sqsubseteq s(e)$.
A typing $s$ is at least as \emph{precise} as another typing $s'$ with $dom(s') \subseteq dom(s)$, written $s \sqsubseteq s'$,
iff for all
expressions $e \in dom(s')$
it holds that $s(e) \sqsubseteq s'(e)$.

For a program $\pi$, the \emph{least precise typesafe typing} $\smin_\pi$ is defined as a minimal typing
where for
every method call $e_0.\PL{m}(e_1,...,e_n)$, $\smin_\pi(e_0) = \bigsqcup \{ t \in \mathcal{T} \mid t \text{ supports method $\PL{m}$ of arity $n$} \}$
and for every conditional or while loop with condition $e$, $\smin_\pi(e) = t_{\mathit{bool}}$.

A typing $s$ for a program $\pi$ is called \emph{consistent} iff it is safe as well as precise enough to
establish type safety: $s \sqsubseteq \smin_\pi$.
By definition, a program is typesafe iff it has a consistent typing\footnote{
if a method call, conditional or while loop is unreachable,
consistent typings may assign the type $\bot$ to its receiver / condition}.


% there are different kinds of typings!
% - flow sensitivity: one mapping [s] < T  vs. one mapping [s] < T for each program location
% - path sensitivity: disjunctions of conjunctions of type literals
% - context sensitivity: one mapping [s] < T per context
% - object sensitivity: like context s. with object contexts

% most concrete typing:
% state-transition system for a program \pi, set of allowed start-states St
% small-step operational semantics defines transition relation (\pi,St) -> (\pi', St')
% addressing: path \pi_0 -> ... -> \pi_n
% states st = function mapping paths \pi_0 -> ... -> \pi_n to the corresponding St
% evaluation: Eval: S x path -> 2^D, Eval(S,p) = V iff (S,st(p)) -*-> (e,St') and \forall \sigma \in St'. \sigma(\result) \in V
% TODO: what about typeerrors, failures, divergence?
% type abstraction: Type: S x path -> T, Type(S,p) = T iff T = |_|_{ v \in Eval(S,p) } \alpha(v)
% typing s = function mapping paths p to \Lamda S. Type(S,p)

% to make s a valid typing:
% for a subexpression S at location l in \pi, s(S) = |_|_{p \in paths(l)} s(S,p)

% this most concrete typing basically evaluates the program itself to determine as precise a type as possible
% for a given expression. Note that the most concrete typing of a program \pi is consistent iff P is typesafe.
% For most programs, however, the most concrete typing is infinite and achieving this level of
% precision hence computationally infeasible.

% From definition 


% More precisely, it is only neccessary to give those subexpressions a type whose result will eventually
% reach a method call or condition. However, all other subexpressions can be removed without affecting the 
% program's behaviour.\todo{neccessary?}

Type inference derives a typing for a given program by
over-approximating its behaviour. A type inference algorithm is \emph{sound}
iff the typings it derives are safe.

% Note that type inference cannot possibly be complete as it would then find consistent
% typings for all typesafe programs and hence decide type safety.

% Note however, that the typings are not necessarily consistent.
% Firstly the program could not be typesafe and secondly deriving consistent typings
% is equivalent to deciding type safety.

Note that given a minimal typing $s$ for a program $\pi$, it is straightforward to decide $s \sqsubseteq \smin_\pi$.
However, deciding safety usually requires more information than contained in a minimal typing.
For this reason, most sound type inference algorithms
a) store more than the minimal type information in their typings and
b) provide a set of inference rules (commonly called a ``type system'')
allowing to check safety of their derived typings using this additional type information.
A soundness proof for these rules with respect to the
semantics of the programming language is a crucial part of proving such algorithms sound.

As the type inference algorithms differ, so do the formats and sizes of their typings. We therefore
associate with each type inference algorithm $\mathit{TI}_X$ a kind of typing $k_X$ capturing the
respective restrictions.

% In Section~\ref{sec:type_inference}, we will exemplary discuss the base case of
% simple algorithm based on a flow-insensitive, path-insensitive and context-insensitive flow-analysis.
% Section~\ref{sec:Extensions} will then discuss more powerful analyses.

Even our simple base-case algorithm already stores one type for every subexpression $S$ of the given
program $\pi$ in its typing. Flow-sensitivity would require additionally storing one type for each
assignment to a variable. Path-sensitivity would require one version of each expressions type for each
path to it from the beginning of its method (which can be exponentially many in the size of the method).
Context-sensitivity would require one version of a method's subexpression's types for each of its contexts.
Here, the number of contexts varies greatly between the number of callsites (program locations where the
method is called) \todo{cite Palsberg}, the number of execution paths that call the method \todo{cite callstring
method} and potentially unbounded in cases of recursive polymorphism.\todo{mention?}


==> sections/variables.tex <==
\begin{definition}
 $change(s) =$
 
 $\{ \PL{u} \mid \PL{u} \text{ appears in an assignment of the form } \PL{u} := e \text{ in } s \} \cup$
 
 $\{ @\PL{v} \mid @\PL{v} \text{ appears in an instance assignment of the form } @\PL{v} := e \text{ in } s \}$
 
 $change(\PL{\textbf{begin local} } \overline{u} := \overline{v}; s \PL{ \textbf{end}}) = change(s) \setminus \{\overline{u}\}$

 $change(\Method) = \bigcup_{C.m \in \Method} change(\PL{\textbf{begin local} } \overline{u} := \overline{v}; s_{C.m} \PL{ \textbf{end}})$

 where $\mathbf{method}\;m(\overline{u})\{s_{C.m}\} \in \Method_C$.
\end{definition}

\begin{definition}
 $var(s) = \{ \PL{u} \mid \PL{u} \text{ appears as a subexpression in } s\}$
\end{definition}

\begin{definition}
 $free(a) = \{ \PL{u} \mid \PL{u} \text{ appears free in } a \}$
\end{definition}


